A Revision of the Mool Language

We present here in a thorough analysis of the Mool language, covering not only its implementation but also the formalisation (syntax, operational semantics, and type system). The objective is to detect glitches in both the implementation and in the formal definitions, proposing as well new features and added expressiveness. To test our proposals we implemented the revision developed in the Racket platform.

==> mool_semantics.tex <==
\begin{figure}
  \textbf{Object Record and Heap Operations}
  \begin{align*}
    \langle C,u,\vec{V}\rangle.f & \defeq \vec{V}(f) &
    \langle C,u,\vec{V}\rangle.\usageterm & \defeq u\\
    \langle C,u,\vec{V}\rangle.\classterm & \defeq C  \\
    \end{align*}
    \textbf{Operations for values and types}
    \begin{align*}
	\linterm(v) & \defeq
                       \begin{cases}
                         tt  & \text{ if } v = o \wedge h(v).\usageterm = \langle u' + u'' \rangle\\
                         tt  & \text{ if } v = o \wedge h(v).\usageterm = \linterm\echoicetypel{m}{z}{i}{I}\\
                         \mathit{ff} &	\text{ otherwise }
                       \end{cases} &
    \unterm(v) & \defeq
                       \begin{cases}
                         tt  & \text{ if } v = \mkterm{unit}\\
                         tt  & \text{ if } v = n\\
                         tt  & \text{ if } v = \true\\
                         tt  & \text{ if } v = \false\\
                         tt  & \text{ if } v = o \wedge h(v).\usageterm = \unterm\echoicetypel{m}{z}{i}{I}\\
                         \mathit{ff} &	\text{ otherwise }
                       \end{cases}
    \end{align*}
   \textbf{Class Definition Operations}
    \begin{align*} 
    C.\methsterm  & \defeq \overrightarrow{M,eval} \quad\text{ where }\class{C}{u}{\vec{F}}{\vec{M}} \in \vec{D} \ \text{and} \ eval \in \{ 0, 1 \}  \\
    C.\fieldsterm  & \defeq \vec{F} \quad\text{ where }\class{C}{u}{\vec{F}}{\vec{M}} \in \vec{D} \\
    C.\usageterm  & \defeq u  \quad\text{ where }\class{C}{u}{\vec{F}}{\vec{M}} \in \vec{D} 
  \end{align*}
  \caption{Auxiliary definitions and Operations}
  \label{fig:aux-defs-oper}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
  \inferrule*[left=R-Context]
  {\stat{h, local}{s_1 \alt \ldots \alt s \alt \ldots \alt s_n}\reduces \stat{h', local'}{s_1 \alt \ldots \alt s' \alt \ldots \alt s_n}}
  {\stat{h, local}{s_1 \alt \ldots \alt \ectx[s] \alt \ldots \alt s_n}\reduces \stat{h', local'}{s_1 \alt \ldots \alt \ectx[s'] \alt \ldots \alt s_n}}
  \and
  \inferrule*[left=R-Spawn]
  {}
  {\stat{h, local}{s_1 \alt \ldots \alt \ectx[\mkterm{spawn}\{s\}] \alt \ldots \alt s_n}\reduces \stat{h, local}{s_1 \alt \ldots \alt \ectx[\mkterm{unit}] \alt \ldots \alt s_n}}
  \end{mathpar}
  \caption{Reduction semantics for states}
  \label{fig:mool_reduc}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
    \inferrule*[left=R-UnField \ ]
    {h(o).f=v\\ \unterm(v,h)}
    {\stat{h,local}{\der{o}{f}} \reduces \stat{h,local}{v}}
    \and
   \inferrule*[left=R-LinField \ ]
   {h(o).f=v\\ \linterm(v,h)}
   {\stat{h,local}{\der{o}{f}} \reduces \stat{\changeval{h}{\der{o}{f}}{\nullterm},local}{v}}
   \and
   \inferrule*[left=R-UnVar \ ]
    {h(d)=v\\ \unterm(v,h)}
    {\stat{h,local}{d} \reduces \stat{h,local}{v}}
    \and
   \inferrule*[left=R-LinVar \ ]
   {h(d)=v\\ \linterm(v,h)}
   {\stat{h,local}{d} \reduces \stat{\changeval{h}{d}{\nullterm},local}{v}}
   \and
    \inferrule*[left=R-Seq \ ]
    {}
    {\stat{h,local}{\seq{v}{s}} \reduces \stat{h,local}{s}} 
    \and
    \inferrule*[left=R-NewVar \ ]
    {}
    {\stat{h,local}{g \ d = v } \reduces \stat{h,\changeval{local}{d}{v}}{\unit}}
    \and
    \inferrule*[left=R-AssignVar \ ]
    {}
    {\stat{h,local}{d = v} \reduces \stat{h,\changeval{local}{d}{v}}{\unit}}
    \and
    \inferrule*[left=R-AssignField \ ]
    {v \neq \nullterm}
    {\stat{h,local}{\upd{o}{f}{v}} \reduces \stat{\changeval{h}{\der{o}{f}}{v},local}{\unit}}
    \and
	 \inferrule*[left=R-AssignFieldNull \ ]
    {v = \nullterm}
    {\stat{h,local}{\upd{o}{f}{v}} \reduces \stat{h \setminus o.f,local}{\unit}}
    \and   
    \inferrule*[left=R-New \ ]
    {o \text{ fresh} \\ (\methodd{\_ }{C}{\_ ~ x}{s}, \_) \in C.\methsterm \\ C.\fieldsterm = \overrightarrow{t~f} \\ C.\usageterm = u }
    {\stat{h,local}{\mkterm{new} \ C(v)}\reduces \stat{(h,o=\langle C, u, \overrightarrow{f=\nullterm}\rangle),local}{s\subs{o}{\this}\subs{v}{x}; o}}
  \and
   \inferrule*[left=R-Call \ ]
   { (\methodd{\_ }{m}{\_ ~ x}{s}, \_) \in (h(o).\classterm).\methsterm  }
   {\stat{h,local}{\selfcal{\der{o}{m}}{v}} \reduces \stat{h,local}{s\subs{o}{\this}\subs{v}{x}}}
  \and
   \inferrule*[left=R-FieldCall \ ]
   { (\methodd{\_ }{m}{\_ ~ x}{s}, \_) \in (h(o).f.\classterm).\methsterm }
   {\stat{h,\varnothing}{\methcal{\der{o}{f}}{m}{v}} \reduces \stat{h,\varnothing}{s\subs{o}{\this}\subs{v}{x}}}
  \and
  \inferrule*[left=R-While \ ]
  {}
  {\stat{h,local}{\while{b}{s}}\reduces \stat{h,local}{\cond{b}{(\seq{s}{\while{b}{s}})}{\unit}}}
  \and
  \inferrule*[left=R-IfTrue \ ]
  {}
  {\stat{h,local}{\cond{\true}{s'}{s''}}\reduces \stat{h,local}{s'}}
 \and
  \inferrule*[left=R-IfFalse \ ]
  {}
  {\stat{h,local}{\cond{\false}{s'}{s''}}\reduces \stat{h,local}{s''}}}
  \end{mathpar}
  \caption{Revised reduction semantics for statements}
  \label{fig:mool_reduc}
\end{figure}

\begin{figure}  
\begin{mathpar}
\mathcal{N} (n)  = n \ \ \ \ \ \ \ \
	\mathcal{A}(n, h, local)  = \mathcal{N}(n) \\
	\mathcal{A}(o.f, h, local)  = h(o).f \ \ \ \ \ \ \ \
	\mathcal{A}(d , h, local)  = local(d) \\
	\mathcal{A}(a_1 + a_2, h, local)  = \mathcal{A} (a_1, h, local) + \mathcal{A} (a_2, h, local) \\
	\mathcal{A}(a_1 - a_2, h, local)  = \mathcal{A} (a_1, h, local) - \mathcal{A} (a_2, h, local)\\
	\mathcal{A}(a_1 * a_2, h, local)  = \mathcal{A} (a_1, h, local) * \mathcal{A} (a_2, h, local) \\ 
	\mathcal{A}(a_1 \ / \ a_2, h, local)  = \mathcal{A} (a_1, h, local) \ / \ \mathcal{A} (a_2, h, local)
\end{mathpar}
  \caption{Evaluation functions for arithmetic values and expressions}
  \label{fig:arith-functions}
\end{figure}

\begin{figure}  
\begin{mathpar}
\mathcal{B}(\true, h, local)  = \true \ \ \ \ \ \ \ \ \mathcal{B}(\false, h, local)  = \false \\ 
\mathcal{B}(o.f, h, local)  = h(o).f  \ \ \ \ \ \ \ \ \mathcal{B}(d , h, local)  = local(d) \\
\mathcal{B}(a_1 == a_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{A} (a_1, h, local) = \mathcal{A} (a_2, h, local) \\
		\false & \mathcal{A} (a_1, h, local) \neq \mathcal{A} (a_2, h, local)		
	\end{cases} \\
\mathcal{B}(a_1 != a_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{A} (a_1, h, local) \neq \mathcal{A} (a_2, h, local) \\
		\false & \mathcal{A} (a_1, h, local) = \mathcal{A} (a_2, h, local)		
	\end{cases} \\
\mathcal{B}(a_1 < a_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{A} (a_1, h, local) < \mathcal{A} (a_2, h, local)\\
		\false & \mathcal{A} (a_1, h, local) >= \mathcal{A} (a_2, h, local)
	\end{cases} \\
\mathcal{B}(a_1 < a_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{A} (a_1, h, local) < \mathcal{A} (a_2, h, local)\\
		\false & \mathcal{A} (a_1, h, local) <= \mathcal{A} (a_2, h, local)
	\end{cases} \\
\mathcal{B}(a_1 <= a_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{A} (a_1, h, local) <= \mathcal{A} (a_2, h, local)\\
		\false & \mathcal{A} (a_1, h, local) > \mathcal{A} (a_2, h, local)
	\end{cases} \\
\mathcal{B}(a_1 >= a_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{A} (a_1, h, local) >= \mathcal{A} (a_2, h, local)\\
		\false & \mathcal{A} (a_1, h, local) < \mathcal{A} (a_2, h, local)
	\end{cases} \\
\mathcal{B}(b_1 \ \&\& \ b_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{B} (b_1, h, local) = \true \wedge (b_2, h, local) = \true \\
		\false & \text{otherwise}
	\end{cases} \\
\mathcal{B}(b_1 \ || \ b_2 , h, local) = 
	\begin{cases} 
		\true & \mathcal{B} (b_1, h, local) = \true \vee (b_2, h, local) = \true \\
		\false & \text{otherwise}
	\end{cases} \\
\mathcal{B}(!b, h, local) = 
	\begin{cases} 
		\true & \mathcal{B} (b, h, local) = \false\\
		\false & \mathcal{B} (b, h, local) = \true
	\end{cases} \\
\end{mathpar}
  \caption{Evaluation functions for boolean values and expressions}
  \label{fig:bool-functions}
\end{figure}

==> mool_type_system.tex <==
\begin{figure}
  \textbf{Type Operations}
  \begin{align*}
  \linterm(t) & \defeq
                       \begin{cases}
                         tt  & \text{ if } v = o \wedge h(v).\usageterm = \langle u' + u'' \rangle\\
                         tt  & \text{ if } v = o \wedge h(v).\usageterm = \linterm\echoicetypel{m}{z}{i}{I}\\
                         \mathit{ff} &	\text{ otherwise }
                       \end{cases}\\
    \unterm(t) & \defeq
                       \begin{cases}
                         tt  & \text{ if } v = \unitterm\\
                         tt  & \text{ if } v = \mkterm{int}\\
                         tt  & \text{ if } v = \boolterm\\
                         tt  & \text{ if } v = o \wedge h(v).\usageterm = \unterm\echoicetypel{m}{z}{i}{I}\\
                         \mathit{ff} &	\text{ otherwise }
                       \end{cases}  \\
       \linterm(\Tenv) & \defeq \forall \ (t \ f) \in \Tenv : \linterm(t)\\
    \unterm(\Tenv) & \defeq \forall \ (t \ f) \in \Tenv : \unterm(t)\\
    \linterm(\vec{F}) & \defeq \forall \ (t \ f) \in \vec{F} : \linterm(t)\\
    \unterm(\vec{F}) & \defeq \forall \ (t \ f) \in \vec{F} : \unterm(t)\\
   \mkterm{check}(\Phi, u) & \defeq
                       \begin{cases}
                       	  \mkterm{check}(\Phi, u_i) &  u = \linterm\echoicetypel{m}{u}{i}{I} \\
                       	  \mkterm{check}(\Phi, u_t) \wedge \mkterm{check}(\Theta, u_f) & u = \langle u_t + u_t \rangle \\
                          \mkterm{check}((\Phi, X : u),u)  & u = \rectype{X}{u} \\
                          \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u_n = \rectype{X}{u_X}\\ 
                          \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u = \linterm\echoicetypel{m}{u}{j}{J}\\ 
                          \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u_n = X \ \wedge \\ & \ \ \ \ \ \  \Phi(X) = \langle u_t + u_t \rangle\\  
                           \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u_n = X \ \wedge \\ & \ \ \ \ \ \  \Phi(X) = \linterm\echoicetypel{m}{u}{j}{J}\\                                  
                          \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u = \langle u_t + u_t \rangle\\                   
                          \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u = \unterm\echoicetypel{m}{u}{j}{J} \wedge m_i \neq m_j\\   
                          \mathit{ff} & u = \unterm\echoicetypel{m}{u}{i}{I} \wedge \exists u_n \in u_i: u_n = X \ \wedge \\ & \ \ \ \ \ \  \Phi(X) = \unterm\echoicetypel{m}{u}{j}{J} \wedge m_i \neq m_j\\                            
                          tt & \text{otherwise}
                       \end{cases}  \\        
    u.\allowsterm(m_j) & \defeq
                       \begin{cases}
                       \epsilon & u = \epsilon \\
                         \unterm  & u=\unterm \\
                         u_j  & u =  \echoicetypel{m}{u}{i}{I} \text{ and } j\in I\\
                         u'\subs{\rectype{X}{u'}}{X}.\allowsterm(m_j)               & u = \rectype{X}{u'}\\
                          \text{undefined} & \text{otherwise}
                       \end{cases}  \\
    \agreeterm(t,t') & \defeq
                       \begin{cases}
                         tt  & \text{ if } t=t'=\booltype\\
                         tt  & \text{ if } t=t'=\mkterm{int}\\
                         tt  & \text{ if } t=t'=\unittype\\
                         tt  & \text{ if } t = \objecttype{C}{u} \text{ and }  t' = \objecttype{C}{u;\vec{F}}\\
                         tt  & \text{ if } t = \mkterm{null} \text{ or }  t' = \mkterm{null}
                       \end{cases}  \\
    \mkterm{modified}(\Tenv, \Tenv') & \defeq
                      \forall r \in \Tenv': \ r \notin \Tenv \vee \Tenv(r) \neq \Tenv'(r)\\
    \mkterm{completed}(\Tenv, \Tenv') & \defeq
                      \forall r \in \Tenv': (r \notin \Tenv \vee \Tenv(r) \neq \Tenv'(r)) \wedge (r = \objecttype{C}{u;\vec{F}} \implies u = \mkterm{un}\{\})
\end{align*}
  \caption{Types, Type Definitions and Operations}
  \label{fig:types-defs}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
   \inferrule*[left=T-Class]
   {\text{check}(\emptyset, u) \\ \objecttype{C}{u;\emptyset} \triangleright u \triangleleft \objecttype{C}{u;\vec{F}} \\ \text{un}(\vec{F})}
   {\typedclass{\class{C}{u}{\vec{F}}{\vec{M}}}}
   \and
   \inferrule*[left=T-UnClass]
   {\forall i\in I \cdot \\\\ %\methodd{\_ }{m}{\_ ~ x}{s}
    (\methodd{y \ t}{m_i}{t'\, x}{s}, \_) \in \vec{M}  \\  \objecttype{C}{\emptyset}, x : t' \triangleright s \triangleleft \objecttype{C}{\vec{F}} \\ \text{un}(\vec{F})}
   {\typedclass{\mkterm{class} \ C \{\vec{F};\vec{M}\}}}  
  \end{mathpar}
  \caption{Revised typing rules for programs}
  \label{fig:mool-typing-programs}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
  \iffalse
   \inferrule*[left=T-BranchEnd \ ]
    % \infrule
    {\forall i\in I \cdot \\\\    
        (\methodd{y \ t}{m}{t'\, x}{s}, \_) \in C.\methsterm  \\
        \typedexp{\this:\objecttype{C}{u;\vec{F}},x:t'}{s}{t}{\Tenv} \\
        \typedval{\Tenv}{\this}{\objecttype{C}{u_i;\vec{F_i}}} \\
    }
    {\Theta; \objecttype{C}{u;\vec{F}}  \triangleright \_ \{m ; un\{\}\} \triangleleft \ \Gamma}
    \fi
   \inferrule*[left=T-Branch \ ]
    % \infrule
    {\forall i\in I \cdot \\\\    
        (\methodd{y \ t}{m_i}{t'\, x}{s}, \_) \in C.\methsterm  \\
        \typedexp{\this:\objecttype{C}{u;\vec{F}},x:t'}{s}{t}{\Tenv} \\\\
        \typedval{\Tenv}{x}{t''} \\ \text{un}(t'') \\
        \typedval{\Tenv}{\this}{\objecttype{C}{u_i;\vec{F_i}}} \\
        \Theta; \Gamma  \triangleright u_i \triangleleft \ \Gamma' 
    }
    {\Theta; \objecttype{C}{u;\vec{F}}  \triangleright \_ \echoicetypel{m}{u}{i}{I} \triangleleft \ \Gamma'}
    \and
    \inferrule*[left=T-BranchEnd \ ]
    % \infrule
    {}
    {\Theta; \Gamma  \triangleright un\{\} \triangleleft \ \Gamma}
    \and
    \inferrule*[left=T-UsageVar \ ]
    % \infrule
    {}
    {(\Theta, X : \Gamma); \Gamma \triangleright X \triangleleft \ \Gamma}
  \end{mathpar}
  \caption{Revised typing rules for usages}
  \label{fig:mool-typing-usages}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
    \inferrule*[left=T-Add \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 + a_2}{\mkterm{int}}{\Tenv''}}
  \and
  \inferrule*[left=T-Sub \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 - a_2}{\mkterm{int}}{\Tenv''}}
  \and
  \inferrule*[left=T-Mult \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 * a_2}{\mkterm{int}}{\Tenv''}}
  \and
  \inferrule*[left=T-Div \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 \ / \ a_2}{\mkterm{int}}{\Tenv''}}
  \end{mathpar}
  \caption{Revised typing rules for arithmetic expressions}
  \label{fig:mool-typing-arith}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
    \inferrule*[left=T-Eq \ ]
  {\typedexp{\Tenv}{e_1}{t}{\Tenv'} \\ \typedexp{\Tenv'}{e_2}{t'}{\Tenv''} \\ \agreeterm(t',t)}
  {\typedexp{\Tenv}{e_1 == e_2}{\mkterm{bool}}{\Tenv''}}
  \and  
  \inferrule*[left=T-Diff \ ]
  {\typedexp{\Tenv}{e_1}{t}{\Tenv'} \\ \typedexp{\Tenv'}{e_2}{t'}{\Tenv''} \\ \agreeterm(t',t)}
  {\typedexp{\Tenv}{e_1 != e_2}{\mkterm{bool}}{\Tenv''}}
  \and
  \inferrule*[left=T-Greater \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 > a_2}{\mkterm{bool}}{\Tenv''}}
  \and
  \inferrule*[left=T-Less \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 < a_2}{\mkterm{bool}}{\Tenv''}}
  \and
  \inferrule*[left=T-GtEqual \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 >= a_2}{\mkterm{bool}}{\Tenv''}}
	\and
	\inferrule*[left=T-LeEqual \ ]
  {\typedexp{\Tenv}{a_1}{\mkterm{int}}{\Tenv'} \\ \typedexp{\Tenv'}{a_2}{\mkterm{int}}{\Tenv''}}
  {\typedexp{\Tenv}{a_1 <= a_2}{\mkterm{bool}}{\Tenv''}}
  \and
  \inferrule*[left=T-And \ ]
  {\typedexp{\Tenv}{b_1}{\mkterm{bool}}{\Tenv'} \\ \typedexp{\Tenv'}{b_2}{\mkterm{bool}}{\Tenv''}}
  {\typedexp{\Tenv}{b_1 \ \&\& \ b_2}{\mkterm{bool}}{\Tenv''}}
  \and
   \inferrule*[left=T-Or \ ]
  {\typedexp{\Tenv}{b_1}{\mkterm{bool}}{\Tenv'} \\ \typedexp{\Tenv'}{b_2}{\mkterm{bool}}{\Tenv''}}
  {\typedexp{\Tenv}{b_1 \ || \ b_2}{\mkterm{bool}}{\Tenv''}}
  \and
   \inferrule*[left=T-Not \ ]
  {\typedexp{\Tenv}{b}{\mkterm{bool}}{\Tenv'}}
  {\typedexp{\Tenv}{!b}{\mkterm{bool}}{\Tenv''}}
  \end{mathpar}
  \caption{Revised typing rules for boolean expressions}
  \label{fig:mool-typing-bool}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
    \inferrule*[left=T-LinVar \ ]
  {\linterm(t)}
  {\typedexp{(\Tenv,r:t)}{r}{t}{\Tenv}}
 \and
 \inferrule*[left=T-UnVar \ ]
  {\unterm(t)}
  {\typedexp{(\Tenv,r:t)}{r}{t}{(\Tenv,r:t)}}
 \and
 \inferrule*[left=T-LinField \ ]
  {\typedval{\Tenv}{this}{\objecttype{C}{u;\vec{F}}} \\ 
   \vec{F}(f)=t \\ \linterm(t) 
 }
  {\typedexp{\Tenv}{\der{\mkterm{this}}{f}}{t}{\changetype{\Tenv}{\mkterm{this}}{\objecttype{C}{u;(\vec{F}\setminus f)}}}} 
 \and
 \inferrule*[left=T-UnField \ ]
  {\typedval{\Tenv}{\mkterm{this}}{\objecttype{C}{u;\vec{F}}} \\ 
  \vec{F}(f)=t
    \\ \unterm(t)}
  {\typedexp{\Tenv}{\der{\mkterm{this}}{f}}{t}{\Tenv}} 
  \end{mathpar}
  \caption{Revised typing rules for field and variable dereference}
  \label{fig:mool-typing-deref}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
	\inferrule*[left=T-AssignVar \ ]
  {e \neq \mkterm{null} \\ \typedexp{\Tenv}{d}{t}{\Tenv'} \\ \typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \agreeterm(t',t)}
  {\typedexp{\Tenv}{d = e}{\unittype}{\Tenv'}}  
	\and
	\inferrule*[left=T-AssignField \ ]
  {e \neq \mkterm{null} \\ \typedexp{\Tenv}{e}{t}{\Tenv'} \\ \typedval{\Tenv'}{\mkterm{this}}{\objecttype{C}{u;\vec{F}}} \\ C.\fieldsterm(f) = t' \\ (t~f) \notin \vec{F} \vee \vec{F}(f) = t' \\ \agreeterm(t',t)}
  {\typedexp{\Tenv}{\upd{\mkterm{this}}{f}{e}}{\unittype}{\changetype{\Tenv'}{\mkterm{this}}{\objecttype{C}{u;(\vec{F}\cup (t~f))}}}}  
	\and
	\inferrule*[left=T-AssignFieldNull \ ]
  {\typedval{\Tenv'}{\mkterm{this}}{\objecttype{C}{u;\vec{F}}} \\ C.\fieldsterm(f) = t}
  {\typedexp{\Tenv}{\upd{\mkterm{this}}{f}{\mkterm{null}}}{\unittype}{\changetype{\Tenv'}{\mkterm{this}}{\objecttype{C}{u;(\vec{F} \setminus (t~f))}}}}  
  \and
  \inferrule*[left=T-NewVar \ ]
  {d \notin \Gamma \\ \typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \agreeterm(t',g)}
  {\typedexp{\Tenv}{g \ d = e}{\unittype}{\changetype{\Tenv'}{d}{g}}} 
  \and
  \inferrule*[left=T-Spawn \ ]
  {\typedexp{\Tenv}{s}{t}{\Tenv'} \\ \unterm(\mkterm{modified}(\Tenv, \Tenv')) \\ \mkterm{completed}(\Tenv, \Tenv')}
  {\typedexp{\Tenv}{\mkterm{spawn} \ \{s\}}{\mkterm{void}}{\Tenv'}}
  \end{mathpar}
  \caption{Revised typing rules for simple statements}
  \label{fig:mool-typing-stms}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
   \inferrule*[left=T-IfCall \ ]
   {w \neq \mkterm{this} \\ \typedexp{\Tenv}{w.m(e)}{\booltype}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{\langle u_t + u_f \rangle ;\vec{F}}} \\ 
   \typedexp{{\changetype{\Tenv'}{w}{\objecttype{C}{u_t;\vec{F}}}}}{s'}{t}{\Tenv''} \\ 
   \typedexp{{\changetype{\Tenv'}{w}{\objecttype{C}{u_f;\vec{F}}}}}{s''}{t}{\Tenv''}}
   {\typedexp{\Tenv}{\cond{w.m(e)}{s'}{s''}}{t}{\Tenv''}} 
   \and
   \inferrule*[left=T-IfNotCall \ ]
   {w \neq \mkterm{this} \\ \typedexp{\Tenv}{w.m(e)}{\booltype}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{\langle u_t + u_f \rangle ;\vec{F}}} \\ 
   \typedexp{{\changetype{\Tenv'}{w}{\objecttype{C}{u_f;\vec{F}}}}}{s'}{t}{\Tenv''} \\ 
   \typedexp{{\changetype{\Tenv'}{w}{\objecttype{C}{u_t;\vec{F}}}}}{s''}{t}{\Tenv''}}
   {\typedexp{\Tenv}{\cond{!w.m(e)}{s'}{s''}}{t}{\Tenv''}} 
   \and
   \inferrule*[left=T-IfUnCall \ ]
   {\typedexp{\Tenv}{w.m(e)}{\booltype}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{\epsilon ;\vec{F}}} \\ 
   \typedexp{\Tenv'}{s'}{t}{\Tenv''} \\ \typedexp{\Tenv'}{s''}{t}{\Tenv''}}
   {\typedexp{\Tenv}{\cond{w.m(e)}{s'}{s''}}{t}{\Tenv''}} 
   \and
   \inferrule*[left=T-If \ ]
   {\typedexp{\Tenv}{b}{\booltype}{\Tenv} \\ \typedexp{\Tenv}{s'}{t}{\Tenv''} \\ \typedexp{\Tenv}{s''}{t}{\Tenv''}}
   {\typedexp{\Tenv}{\cond{b}{s'}{s''}}{t}{\Tenv''}} 
   \and
  \and
   \inferrule*[left=T-WhileCall \ ]
   {w \neq \mkterm{this} \\ \typedexp{\Tenv}{w.m(e)}{\booltype}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{\langle u_t + u_f \rangle ;\vec{F}}} \\ 
    \typedexp{{\changetype{\Tenv'}{w}{\objecttype{C}{u_t;\vec{F}}}}}{s'}{t}{\Tenv''} \\ \Tenv(w) = \Tenv''(w)}
   {\typedexp{\Tenv}{\while{w.m(e)}{s'}}{t}{\changetype{\Tenv''}{w}{\objecttype{C}{u_f;\vec{F}}}}}  
   \and
   \inferrule*[left=T-WhileNotCall \ ]
   {w \neq \mkterm{this} \\ \typedexp{\Tenv}{w.m(e)}{\booltype}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{\langle u_t + u_f \rangle ;\vec{F}}} \\ 
    \typedexp{{\changetype{\Tenv'}{w}{\objecttype{C}{u_f;\vec{F}}}}}{s'}{t}{\Tenv''} \\ \Tenv(w) = \Tenv''(w)}
   {\typedexp{\Tenv}{\while{!w.m(e)}{s'}}{t}{\changetype{\Tenv''}{w}{\objecttype{C}{u_t;\vec{F}}}}}  
   \and
   \inferrule*[left=T-WhileUnCall \ ]
   {\typedexp{\Tenv}{w.m(e)}{\booltype}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{\epsilon ;\vec{F}}} \\ 
    \typedexp{\Tenv'}{s}{t}{\Tenv} \\ }
   {\typedexp{\Tenv}{\while{w.m(e)}{s}}{t}{\Tenv'}}  
   \and
  \inferrule*[left=T-While \ ]
   {\typedexp{\Tenv}{b}{\booltype}{\Tenv} \\ \typedexp{\Tenv}{s}{t}{\Tenv}}
   {\typedexp{\Tenv}{\while{b}{s}}{t}{\Tenv}}  
  \end{mathpar}
  \caption{Revised typing rules for control flow expressions}
  \label{fig:mool-typing-flow}
\end{figure}

\begin{figure}
  \centering
  \begin{mathpar}
  \inferrule*[left=T-New]
  {\typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \\  C.\usageterm = \mkterm{lin}\{C; u\} \\ (\methodd{t}{C}{t'\, x}{s}, \_) \in C.\methsterm \\ \unterm(\Tenv' \backslash \Tenv)}
  {\typedexp{\Tenv}{\mkterm{new} \ C (e)}{\objecttype{C}{u}}{\Tenv'}}
  \and
  \inferrule*[left=T-UnNew]
  {\typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \\  C.\usageterm = \epsilon \\ (\methodd{t}{C}{t'\, x}{s}, \_) \in C.\methsterm \\ \unterm(\Tenv' \backslash \Tenv)}
  {\typedexp{\Tenv}{\mkterm{new} \ C (e)}{\objecttype{C}{u}}{\Tenv'}}
  \and
      \inferrule*[left=T-SelfCall1 \ ]
  	{\typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \typedval{\Tenv'}{\this}{\objecttype{C}{u;\vec{F}}}\\ (\methodd{t}{m}{t'\, x}{s}, 0) \in C.\methsterm \\ \typedexp{\Tenv'}{s}{t}{\Tenv''} \\ \unterm(\Tenv' \backslash \Tenv)}  
  {\typedexp{\Tenv}{\methcal{\this}{m}{e}}{t}{\Tenv''}}
\and
      \inferrule*[left=T-SelfCall2 \ ]
  	{\typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \typedval{\Tenv'}{\this}{\objecttype{C}{u;\vec{F}}}\\ (\methodd{t}{m}{t'\, x}{s}, 1) \in C.\methsterm}  
  {\typedexp{\Tenv}{\methcal{\this}{m}{e}}{t}{\Tenv'}}
\and
   \inferrule*[left=T-Call \ ]
  {w \neq \mkterm{this} \\ \typedexp{\Tenv}{e}{t'}{\Tenv'} \\ \typedval{\Tenv'}{w}{\objecttype{C}{u;\vec{F}}}\\  u.\allowsterm(m)= u'  \\ (\methodd{t}{m}{t'\, x}{s}, \_) \in C.\methsterm \\ \unterm(\Tenv' \backslash \Tenv)}
  {\typedexp{\Tenv}{\methcal{w}{m}{e}}{t}{\changetype{\Tenv'}{w}{\objecttype{C}{u';\vec{G}}}}}
  \end{mathpar}
  \caption{Revised typing rules for calls}
  \label{fig:mool-typing-calls}
\end{figure}

==> useful-macros.tex <==
% Colours

\usepackage{color}
\definecolor{dkblue}{rgb}{0,0.1,0.5}
\definecolor{dkgreen}{rgb}{0,0.4,0}
\def\Red{\color{\ifdraft red\else black\fi}}
\def\Green{\color{\ifdraft green\else black\fi}}
\def\Blue{\color{\ifdraft blue\else black\fi}}
\def\Black{\color{black}}
\newcommand{\details}[1]{\iffull{\Blue#1}\fi}
\definecolor{linkColor}{rgb}{0,0,0.5}

% Theorems etc.
\makeatletter
\@ifclassloaded{beamer}
  {\relax}
  {\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}

\newtheorem{saetning}{S{\ae}tning}
\newtheorem{proposition}{Proposition}
\newtheorem{korollar}{Korollar}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{eksempel}{Eksempel}
\newtheorem{exercise}{Exercise}
\newtheorem{problem}[theorem]{Problem}}
\makeatother
\newenvironment{bevis}{\begin{proof}[Bevis:]}{\end{proof}}

\input{commands}

==> useful-packages.tex <==
% Common packages

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{listings}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{stmaryrd}
\usepackage{tikz}

